ICE: Intrinsic Concept Extraction from a Single Image via Diffusion Models

The inherent ambiguity in defining visual concepts poses significant challenges for modern generative models, such as the diffusion-based Text-to-Image (T2I) models, in accurately learning concepts from a single image. Existing methods lack a systematic way to reliably extract the interpretable underlying intrinsic concepts. To address this challenge, we present ICE, short for Intrinsic Concept Extraction, a novel framework that exclusively utilises a T2I model to automatically and systematically extract intrinsic concepts from a single image. ICE consists of two pivotal stages. In the first stage, ICE devises an automatic concept localization module to pinpoint relevant text-based concepts and their corresponding masks within the image. This critical stage streamlines concept initialization and provides precise guidance for subsequent analysis. The second stage delves deeper into each identified mask, decomposing the object-level concepts into intrinsic concepts and general concepts. This decomposition allows for a more granular and interpretable breakdown of visual elements. Our framework demonstrates superior performance on intrinsic concept extraction from a single image in an unsupervised manner. Project page: https://visual-ai.github.io/ice

==> macros.tex <==
% \usepackage{xcolor}
% \usepackage{wrapfig}
% \usepackage{soul}

% \definecolor{yellow}{rgb}{1,1, 0.6}
% \definecolor{lightyellow}{rgb}{1,1, 0.8}
% \definecolor{orange}{rgb}{1, 0.8, 0.6}
% \definecolor{coral}{RGB}{246,131,65}
% \definecolor{pinkred}{rgb}{1, 0.6, 0.6}
% \definecolor{hotpink}{RGB}{238,64,195}
% \definecolor{lavender}{RGB}{207,226,243}
% \definecolor{gainsboro}{RGB}{208,224,227}
% \definecolor{gainsboro2}{RGB}{217,234,211}
% \definecolor{blanchedalmond}{RGB}{252,229,205}

% \newcommand{\missfigure}{\textcolor{red}{[F]}}
% \newcommand{\misscite}{\textcolor{red}{[C]}}
% \newcommand{\missref}{\textcolor{red}{[R]}}

% \newcommand{\ray}[1]{{\textcolor{red}{#1}}}
% \newcommand{\todo}[1]{{\textcolor{red}{(TODO: #1)}}}

% \newcommand{\model}{XXXX}
% \newcommand{\modelname}{XXXX\xspace}

% \newcommand{\coverage}{spatial coverage\xspace}
% \newcommand{\complexity}{detail complexity\xspace}
% %altitude or distance
% \newcommand{\altitude}{distance\xspace}
% \newcommand{\altitudefull}{distance to the scene\xspace}
% \newcommand{\altitudes}{distances\xspace}
% \newcommand{\altitudesfull}{distances to the scene\xspace}
